Asymptotic normality and combinatorial aspects of the prefix exchange distance distribution

The prefix exchange distance of a permutation is the minimum number of exchanges involving the leftmost element that sorts the permutation. We give new combinatorial proofs of known results on the distribution of the prefix exchange distance for a random uniform permutation. We also obtain expressions for the mean and the variance of this distribution, and finally, we show that the normalised prefix exchange distribution converges in distribution to the standard normal distribution.

==> newtheorems-en.tex <==
\RequirePackage{amsthm} % for \theoremstyle
\theoremstyle{definition} % causes definitions to be typeset normally, emphasizing only the defined term
\newtheorem{definition}{Definition}[section]
\theoremstyle{plain} % switch back to the default theorem style

\newtheorem{proposition}{Proposition}[section]

\newtheorem{example}{Example}[section]
\newtheorem{fact}{Fact}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{observation}{Observation}[section]
\newtheorem{conjecture}{Conjecture}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{theorem}{Theorem}[section]


